Hierarchical Attention Generates Better Proofs

Large language models (LLMs) have shown promise in formal theorem proving, but their token-level processing often fails to capture the inherent hierarchical nature of mathematical proofs. We introduce \textbf{Hierarchical Attention}, a regularization method that aligns LLMs' attention mechanisms with mathematical reasoning structures. Our approach establishes a five-level hierarchy from foundational elements to high-level concepts, ensuring structured information flow in proof generation. Experiments demonstrate that our method improves proof success rates by 2.05\% on miniF2F and 1.69\% on ProofNet while reducing proof complexity by 23.81\% and 16.50\% respectively. The code is available at https://github.com/Car-pe/HAGBP.

==> sections/04_methods_axioms.tex <==
\section{Approach}

\subsection{Overview}

Mathematical theorem proving requires precise understanding of hierarchical relationships between concepts. Although large language models have shown promising results in this domain, their attention mechanisms often fail to capture these inherent mathematical structures. We address this challenge through a principled framework that enforces hierarchical attention patterns while preserving the model's reasoning capabilities.

\begin{figure}[t]
\centering
[Insert overview diagram]
\caption{Overview of our hierarchical attention framework. Mathematical statements are parsed into semantic levels (e.g., definitions $\rightarrow$ conditions $\rightarrow$ goals), which guide attention patterns through our axiomatic framework while maintaining flexibility for complex reasoning.}
\label{fig:overview}
\end{figure}

Our key insight is that mathematical statements naturally decompose into hierarchical levels, and this structure should guide the model's attention patterns. We formalize this intuition through an axiomatic framework that characterizes essential properties of hierarchical attention, leading to a provably unique solution. 

\subsection{Notation and Preliminaries}

We first introduce the key notation and concepts used throughout this section.

\paragraph{Basic Notation.} Let $\mathcal{T}$ denote the input theorem text and $T$ be the set of all tokens. We use $t_i, t_j$ to denote individual tokens, $L$ for the number of transformer layers, and $l \in [1,L]$ for layer indices.

\paragraph{Level Assignment.} Each token is assigned to one of five hierarchical levels $T_k$ where $k \in \{0,1,2,3,4\}$, corresponding to different components in theorem proving:
\begin{itemize}
    \item $T_0$ (other): External content such as prompts and comments
    \item $T_1$ (case): Theorem names and case statements
    \item $T_2$ (type): Type declarations and definitions
    \item $T_3$ (instance): Instance declarations and concrete examples
    \item $T_4$ (goal): The final proof goal to be established
\end{itemize}
The function $\text{level}(t)$ returns the hierarchical level ($0,1,2,3,4$) of token $t$. We use $f(s)$ to denote the feature extraction function that extracts pattern features from sequence $s$, and $\text{ClassifyLevel}(f)$ assigns levels based on these features. This hierarchical structure naturally reflects the dependency flow in mathematical reasoning, where higher levels build upon the foundations established in lower levels.

\paragraph{Attention Mechanism.} The attention score from token $x$ to token $y$ in layer $l$ is denoted as $att_l(x,y)$. The binary attention mask between tokens $i$ and $j$ is represented by $M_{ij}$, where $M_{ij} = 1$ indicates allowed attention flow and $M_{ij} = 0$ indicates prohibited attention that will be penalized by our loss function. The attention loss is denoted as $\mathcal{L}_{att}$, with $\mathcal{L}_{att}^l$ representing layer-specific loss. When attention flows violate the mask (i.e., $att_l(x,y) > 0$ when $M_{xy} = 0$), they are penalized through the loss computation.

\paragraph{Semantic Relations.} We use $\prec$ to denote the partial order relation between levels (e.g., $other \prec case$ means "other" is lower than "case"). The semantic dependency relation $\text{dep}(x,y)$ indicates token $x$ depends on token $y$. The semantic content of a token is denoted by $sem(t)$, and $\approx$ represents similarity between pattern features.




\subsection{Hierarchical Information Flow}

We begin by establishing four fundamental axioms that characterize our hierarchical attention mechanism. These axioms form the theoretical foundation of our approach and lead to provable properties about the behavior of our system.


\begin{axiom}[Information flow order]
The attention mechanism must preserve the hierarchical structure:
\[
\text{level}(t_i) \leq \text{level}(t_j) \iff M_{ij} = 1
\]
where $M_{ij}$ is the attention mask that enforces the partial order: $other \prec case \prec type \prec instance \prec goal$.
\end{axiom}

\begin{axiom}[Sensitivity]
If a token $x$ depends semantically on token $y$, then the attention mechanism must reflect this dependency:
\[
\text{dep}(x,y) \implies \exists l: \text{att}_l(x,y) > 0
\]
This guarantees that all mathematical dependencies are captured in the attention patterns.
\end{axiom}

\begin{axiom}[Completeness]
Every token must be assigned exactly one hierarchical level, and every token pair must have a defined mask value:
\[
 \forall t \in T: \exists! k \in \{0,1,2,3,4\}: t \in T_k 
\]
This ensures that the hierarchical structure is well-defined for all tokens in the input.
\end{axiom}



% \begin{theorem}[Level Assignment Consistency]
% Given Implementation Invariance and Completeness axioms, for any tokens $x, y$:
% \begin{equation}
% f(x) = f(y) \implies \exists! k \in \{0,1,2,3,4\}: x,y \in T_k
% \end{equation}
% \end{theorem}

% \begin{proof}
% Let $x, y$ be any tokens where $f(x) = f(y)$.

% 1. By Completeness axiom:
% \[
% \exists! k_1 \in \{0,1,2,3,4\}: x \in T_{k_1}
% \]
% \[
% \exists! k_2 \in \{0,1,2,3,4\}: y \in T_{k_2}
% \]

% 2. By Implementation Invariance:
% \[
% f(x) = f(y) \implies \text{level}(x) = \text{level}(y)
% \]

% 3. Since $\text{level}(x) = k_1$ and $\text{level}(y) = k_2$:
% \[
% k_1 = k_2 = k
% \]

% 4. Therefore:
% \[
% \exists! k \in \{0,1,2,3,4\}: x,y \in T_k
% \]
% \end{proof}

\begin{theorem}[Hierarchical Attention Flow]
Given Structural Preservation and Sensitivity axioms, for any tokens $x, y$, the following implications hold:

From semantic dependency to hierarchical levels:
\begin{equation}
\begin{aligned}
\text{dep}(x,y) & \implies \exists l: att_l(x,y) > 0 \\
& \implies M_{xy} = 1 \\
& \implies \text{level}(x) \leq \text{level}(y)
\end{aligned}
\end{equation}
\end{theorem}

\begin{proof}
We prove each implication chain:

\textbf{Part (1):}
1. Given $\text{level}(x) \leq \text{level}(y)$
2. By Structural Preservation:
\[
\text{level}(x) \leq \text{level}(y) \iff M_{xy} = 1
\]

\textbf{Part (2):}
1. Given $\text{dep}(x,y)$
2. By Sensitivity:
\[
\text{dep}(x,y) \implies \exists l: att_l(x,y) > 0
\]

3. By construction of our attention mechanism:
\[
att_l(x,y) > 0 \implies M_{xy} = 1
\]
This implication holds because:
\begin{itemize}
    \item When $M_{xy} = 0$, our loss function computes:
    \[
    invalid_{att} = att_l(x,y) \cdot (1 - M_{xy}) = att_l(x,y)
    \]
    \item The loss penalizes any positive $invalid_{att}$ through:
    \[
    penalties = \text{ReLU}(invalid_{att})
    \]
    \item Therefore, at convergence, $att_l(x,y)$ must be 0 when $M_{xy} = 0$
    \item Equivalently, $att_l(x,y) > 0$ implies $M_{xy} = 1$
\end{itemize}

4. By Structural Preservation:
\[
M_{xy} = 1 \iff \text{level}(x) \leq \text{level}(y)
\]

This establishes both parts of the theorem.
\end{proof}

These theorems establish the consistency and correctness of our hierarchical attention mechanism, showing that it properly captures both pattern-based level assignments and semantic dependencies in the input. This theoretical foundation provides strong guarantees about the behavior of our system, which we implement efficiently through attention masking and loss computation as detailed in the following sections.





\subsection{Algorithm}
We now present an algorithm that systematically implements these axioms and properties. The algorithm constructs a hierarchical structure that provably satisfies our theoretical requirements.

\begin{algorithm}
\caption{Hierarchical Attention Mechanism}
\KwIn{Theorem text $\mathcal{T}$}
\KwOut{Hierarchical structure and attention mask $M$}
\BlankLine
\tcc{Initialize for Structural Preservation}
Initialize level sets $\{T_0, T_1, T_2, T_3, T_4\}$ following partial order\;
Initialize pattern-based classifier $\mathcal{C}$\;
\BlankLine
\For{each sequence $s$ in $\mathcal{T}$}{
    \tcc{Implementation Invariance through pattern-based classification}
    Parse sequence $s$ into tokens\;
    Extract semantic features $f(s)$ using predefined patterns\;
    $l \gets \text{ClassifyLevel}(f(s))$ according to partial order\;
    Add tokens to corresponding level $T_l$\;
}
\BlankLine
\tcc{Structural Preservation through mask construction}
\For{tokens $i,j$ in input sequence}{
    $M_{ij} \gets \mathbf{1}[\text{level}(t_i) \leq \text{level}(t_j)]$\;
}
\BlankLine
\Return{Level assignments and attention mask $M$}\;
\end{algorithm}

The algorithm directly implements our axioms:
\begin{itemize}
    \item Implementation Invariance is ensured through consistent feature-based classification
    \item Sensitivity is maintained by explicit dependency tracking
    \item Completeness is guaranteed by comprehensive level assignment
    \item Structural Preservation is enforced through semantic verification and mask construction
\end{itemize}

This algorithmic framework provides the foundation for our attention mechanism, which we implement through masking and loss computation as detailed in the following section.

\subsection{Implementation}

The implementation of our approach centers on two key components that work together to enforce our axioms while maintaining computational efficiency: attention masking and loss computation.

\subsubsection{Attention Masking}
We implement the structural constraints through a hierarchical attention mask:
\begin{equation}
M_{ij} = \begin{cases}
    1 & \text{if } level(t_i) \leq level(t_j) \\
    0 & \text{otherwise}
\end{cases}
\end{equation}

This mask directly enforces the Structural Preservation axiom by ensuring that attention flows only from lower to higher or equal levels, while maintaining the partial order established in Section 3.2.

\subsubsection{Loss Computation}
The attention loss is designed to enforce our axioms while allowing flexible reasoning:

\begin{algorithm}
\caption{Attention Loss Computation}
\KwIn{Attention scores $\{att_l\}_{l=1}^L$, Input tokens $T$}
\KwOut{Attention loss $\mathcal{L}_{att}$}
Parse input tokens to get hierarchical levels\;
Initialize $\mathcal{L}_{att} \gets 0$\;
\For{each layer $l$ in $1$ to $L$}{
    Compute mask violations: $invalid_{att} \gets att_l \cdot (1 - M)$\;
    $penalties \gets \text{ReLU}(invalid_{att})$\;
    \tcc{Layer-wise adaptation for flexible reasoning}
    $\mathcal{L}_{att}^l \gets (1 - l/L) \cdot \sum penalties$\;
    $\mathcal{L}_{att} \gets \mathcal{L}_{att} + \mathcal{L}_{att}^l$\;
}
$\mathcal{L}_{att} \gets \mathcal{L}_{att}/|T|$\;
\Return{$\mathcal{L}_{att}$}\;
\end{algorithm}

Our loss function incorporates layer-wise adaptation through a depth-dependent scaling factor $(1 - \frac{l}{L})$, which allows the model to balance between strict hierarchical adherence in lower layers and more flexible reasoning patterns in higher layers. The final loss is normalized by sequence length to ensure consistent scaling across different inputs. This formulation provides a principled way to enforce our theoretical constraints while maintaining the model's capacity for complex mathematical reasoning.

\begin{figure}[h]
\centering
[Insert visualization showing attention patterns with and without our hierarchical constraints]
\caption{Impact of hierarchical attention constraints. Left: Standard attention patterns. Right: Attention patterns with our constraints, showing clear hierarchical structure while maintaining flexibility for complex reasoning.}
\label{fig:attention_patterns}
\end{figure}



\subsection{Uniqueness}
We now establish that our approach is not merely one possible solution, but the unique solution satisfying our axiomatic requirements. This uniqueness result provides strong theoretical justification for our algorithm design.

\begin{theorem}[Uniqueness of Hierarchical Attention]
Any attention mechanism satisfying our four axioms must be structurally equivalent to our algorighm.
\end{theorem}

\begin{proof}
Let $\mathcal{A}$ be any algorithm satisfying our axioms. We prove uniqueness through two steps:

\textbf{Step 1: Level Assignment Uniqueness}

First, we prove that any valid level assignment must be identical to the one produced by our algorithm. Consider any sequence $s$ in the input theorem text $\mathcal{T}$:

\begin{itemize}
    \item By Implementation Invariance:
    \[
    f(s_1) = f(s_2) \implies \text{level}(s_1) = \text{level}(s_2)
    \]
    Therefore, the level assignment must be determined solely by the pattern features $f(s)$.
    
    \item By Completeness:
    \[
    \forall t \in T: \exists! k \in \{0,1,2,3,4\}: t \in T_k
    \]
    Each token must be assigned to exactly one level.
    
    \item By Structural Preservation and the partial order:
    \[
    other \prec case \prec type \prec instance \prec goal
    \]
    The level assignment must respect this hierarchical structure.
\end{itemize}

These constraints uniquely determine the level assignment function:
\[
\text{level}_{\mathcal{A}}(s) = \text{ClassifyLevel}(f(s))
\]
which matches Algorithm 1's implementation.

\textbf{Step 2: Attention Pattern Uniqueness}

Given the unique level assignment, we prove that the attention patterns must also be uniquely determined:

\begin{itemize}
    \item By Structural Preservation:
    \[
    \text{level}(t_i) \leq \text{level}(t_j) \iff M_{ij} = 1
    \]
    This uniquely determines the mask structure.
    
    \item By Sensitivity and Hierarchical Attention Flow:
    \[
    \text{dep}(x,y) \implies \exists l: att_l(x,y) > 0 \implies M_{xy} = 1
    \]
    This ensures necessary attention paths are preserved.
    
    \item By Completeness:
    \[
    \forall t_i, t_j \in T: \exists M_{ij} \in \{0,1\}
    \]
    The mask is well-defined for all token pairs.
\end{itemize}

These conditions uniquely determine the attention mask:
\[
M_{ij} = \begin{cases}
    1 & \text{if } \text{level}(t_i) \leq \text{level}(t_j) \\
    0 & \text{otherwise}
\end{cases}
\]

Therefore, any algorithm $\mathcal{A}$ satisfying our axioms must:
\begin{enumerate}
    \item Produce identical level assignments through pattern-based classification
    \item Generate identical attention masks through level-based constraints
\end{enumerate}

This establishes the structural uniqueness of our approach.
\end{proof}
This uniqueness result, combined with our efficient implementation through attention masking and loss computation, establishes our method as the canonical solution for hierarchical attention in theorem proving.

==> sections/04_methods_old.tex <==
\section{Approach}
\subsection{Hierarchical Parsing System}

We introduce a novel category-theoretic framework for parsing mathematical theorems that bridges the gap between syntactic structure and semantic interpretation. Our key insight is that mathematical statements naturally form a categorical structure that can guide attention mechanisms in neural networks.

\subsubsection{Theoretical Foundation}

Let $\mathcal{H}$ be the category of hierarchical token structures where:
\begin{itemize}
\item Objects are token sequences $Obj(\mathcal{H}) = \{T_l | l \in \{0,1,2,3,4\}\}$, representing five semantic levels
\item Morphisms $Mor(T_i, T_j)$ represent valid hierarchical transitions with semantic preservation
\item Composition satisfies the axiom: $f \circ g \in Mor(T_i, T_k)$ for $f \in Mor(T_j, T_k)$, $g \in Mor(T_i, T_j)$
\end{itemize}

The hierarchy induces a strict partial order with semantic constraints:
\begin{equation}
other \prec case \prec type \prec instance \prec goal
\end{equation}

This ordering satisfies two key properties that guide our parsing algorithm:

\begin{theorem}[Semantic Preservation]
For any morphism $f: T_i \to T_j$:
\begin{equation}
sem(T_j) \subseteq sem(T_i) \text{ where } sem(T) \text{ denotes semantic content}
\end{equation}
This ensures that higher-level tokens maintain semantic consistency with their dependencies.
\end{theorem}

\begin{theorem}[Hierarchical Completeness]
For any tokens $x, y$:
\begin{equation}
x \text{ depends on } y \Rightarrow \exists f \in Mor(T_i, T_j): f(x) \text{ relates to } y
\end{equation}
This guarantees that all semantic dependencies are captured by morphisms in our category.
\end{theorem}

\subsubsection{Algorithmic Framework}

Based on these theoretical foundations, we develop an algorithm that implements the categorical structure while ensuring our theoretical guarantees:

\begin{algorithm}
\caption{Hierarchical Theorem Parsing}
\begin{algorithmic}[1]
\REQUIRE Theorem text $\mathcal{T}$
\ENSURE Hierarchical structure $\mathcal{H}$ satisfying categorical properties
\STATE // Initialize category $\mathcal{H}$ with objects and morphisms
\STATE Initialize objects $Obj(\mathcal{H}) = \{T_0, T_1, T_2, T_3, T_4\}$ 
\STATE Initialize morphism sets $Mor(T_i, T_j) = \emptyset$ for all $i \leq j$
\FOR{each sequence $s$ in $\mathcal{T}$}
    \STATE // Pattern-based classification respecting partial order
    \STATE $l \gets \text{ClassifyLevel}(s)$ according to $other \prec case \prec type \prec instance \prec goal$
    \STATE Add $s$ to object $T_l$
    \STATE // Create and verify morphisms (Semantic Preservation)
    \FOR{$i < l$}
        \STATE $f_{il} \gets \text{CreateMorphism}(T_i, T_l)$
        \STATE Assert $sem(T_l) \subseteq sem(T_i)$ \COMMENT{Theorem 4.1: Semantic Preservation}
        \STATE Add $f_{il}$ to $Mor(T_i, T_l)$
        \STATE // Ensure composition axiom
        \FOR{$k < i$}
            \STATE $f_{kl} \gets f_{ki} \circ f_{il}$
            \STATE Add $f_{kl}$ to $Mor(T_k, T_l)$
        \ENDFOR
    \ENDFOR
\ENDFOR
\STATE // Verify Hierarchical Completeness (Theorem 4.2: Dependency Preservation)
\FOR{each pair of tokens $(x,y)$ with dependency}
    \STATE Find levels $i,j$ where $x \in T_i, y \in T_j$
    \STATE Assert $\exists f \in Mor(T_i, T_j)$ relating $x$ to $y$
\ENDFOR
\STATE \textbf{return} $\mathcal{H}$
\end{algorithmic}
\end{algorithm}

\subsubsection{Theoretical Guarantees}

Our algorithm explicitly enforces three critical guarantees through its implementation:

1. \textbf{Structural Soundness}: The parsing preserves mathematical dependencies through morphism verification (Lines 10-11):
\begin{equation}
\forall x, y \in \mathcal{T}: dep(x,y) \Rightarrow level(x) \geq level(y)
\end{equation}

2. \textbf{Semantic Coherence}: Token classifications respect semantic relationships through the composition axiom (Lines 13-16):
\begin{equation}
\forall f \in Mor(T_i, T_j): sem(cod(f)) \text{ refines } sem(dom(f))
\end{equation}

3. \textbf{Completeness}: Every token receives a valid classification through the initialization and main loop (Lines 1-8):
\begin{equation}
\forall t \in \mathcal{T}: \exists l \in \{0,\ldots,4\}: t \in T_l
\end{equation}

These guarantees, when implemented through our algorithm, ensure that the attention mechanisms in our neural model respect the inherent mathematical structure of theorems, leading to improved proof generation (see Section \ref{sec:experiments}).

\subsection{Categorical Structure of Attention and Loss}

We formalize the attention mechanism and its associated loss through a structure-preserving functor $F: \mathcal{H} \rightarrow \mathcal{A}$ between the hierarchical token category $\mathcal{H}$ and the attention category $\mathcal{A}$. This formulation enables both principled control over attention patterns and theoretically grounded loss computation.

\subsubsection{Functorial Properties}

The functor $F$ satisfies three key properties that guide our attention mechanism design:

1. \textbf{Composition Preservation}:
\begin{equation}
\begin{aligned}
& \forall f \in Hom_{\mathcal{H}}(A,B), g \in Hom_{\mathcal{H}}(B,C): \\
& F(f \circ g) = F(f) \circ F(g) \in Hom_{\mathcal{A}}(F(A),F(C))
\end{aligned}
\end{equation}
This property ensures that attention patterns respect hierarchical relationships across multiple levels.

2. \textbf{Order Preservation}:
\begin{equation}
\begin{aligned}
& \forall a,b \in Ob(\mathcal{H}): \\
& a \leq_{\mathcal{H}} b \implies F(a) \leq_{\mathcal{A}} F(b)
\end{aligned}
\end{equation}
This directly translates to our hierarchical masking mechanism in the attention computation.

3. \textbf{Structural Isomorphism}:
\begin{equation}
\begin{aligned}
& \exists \eta: 1_{\mathcal{H}} \Rightarrow F^{op}F, \epsilon: FF^{op} \Rightarrow 1_{\mathcal{A}} \\
& \text{such that } (\epsilon F) \circ (F\eta) = 1_F
\end{aligned}
\end{equation}
This ensures that our attention transformation preserves the essential structure of the input.

\subsubsection{Attention Pattern Control and Loss}

These categorical properties are implemented through our attention mechanism and loss computation:

\begin{algorithm}[h]
\caption{Categorical Attention Loss Computation}
\begin{algorithmic}[1]
\REQUIRE Attention scores $\{att_l\}_{l=1}^L$, Input tokens $T$
\ENSURE Attention loss $\mathcal{L}_{att}$
\STATE // Initialize based on structural isomorphism
\STATE Parse input tokens to get hierarchical levels
\STATE Initialize total loss $\mathcal{L}_{att} \gets 0$
\FOR{each layer $l$ in $1$ to $L$}
    \STATE // Implement order preservation through masking
    \FOR{tokens $i,j$ in input sequence}
        \STATE $M_{ij} \gets \mathbf{1}[level(t_i) \leq level(t_j)]$
    \ENDFOR
    \STATE // Enforce composition preservation
    \STATE $invalid_{att} \gets att_l \cdot (1 - M)$
    \STATE $penalties \gets \text{ReLU}(invalid_{att})$
    \STATE // Layer-wise adaptation for flexible reasoning
    \STATE $depth\_factor \gets 1 - l/L$
    \STATE $\mathcal{L}_{att}^l \gets depth\_factor \cdot \sum penalties$
    \STATE // Accumulate loss while maintaining structure
    \STATE $\mathcal{L}_{att} \gets \mathcal{L}_{att} + \mathcal{L}_{att}^l$
\ENDFOR
\STATE // Normalize while preserving relative relationships
\STATE $\mathcal{L}_{att} \gets \mathcal{L}_{att}/|T|$
\STATE \textbf{return} $\mathcal{L}_{att}$
\end{algorithmic}
\end{algorithm}

The algorithm implements our theoretical framework through three key components that directly correspond to our functorial properties:

1. \textbf{Hierarchical Masking} (Lines 5-7): Implements order preservation through the mask:
\begin{equation}
M_{ij} = \begin{cases}
    1 & \text{if } level(t_i) \leq level(t_j) \\
    0 & \text{otherwise}
\end{cases}
\end{equation}

2. \textbf{Layer-wise Attention Loss} (Lines 12-14): Enforces composition preservation:
\begin{equation}
\mathcal{L}_{att}^l = (1 - \frac{l}{L}) \sum_{i,j} \text{ReLU}(att_{l,i,j} \cdot (1 - M_{ij}))
\end{equation}

3. \textbf{Total Loss} (Lines 15-19): Maintains structural isomorphism:
\begin{equation}
\mathcal{L}_{att} = \frac{1}{|T|} \sum_{l=1}^L \mathcal{L}_{att}^l
\end{equation}

As illustrated in Figure \ref{fig:parser}, this implementation yields two key advantages:

\begin{itemize}
\item \textbf{Structural Coherence}: The functor $F$ ensures that attention patterns respect the inherent hierarchical structure of mathematical statements, as implemented through our masking mechanism
\item \textbf{Adaptive Constraint}: The layer-wise loss formulation provides a principled way to balance between strict hierarchical adherence and flexible attention patterns, achieved through our depth-dependent scaling
\end{itemize}

This formulation bridges the gap between categorical abstraction and practical attention control, providing both theoretical guarantees and an efficient implementation.


\subsection{Axiomatic Characterization and Uniqueness}

We present an axiomatic characterization of hierarchical attention mechanisms and prove that our algorithm is the unique solution satisfying these axioms. This approach follows the tradition of axiomatic attribution methods in deep learning.

\subsubsection{Axioms for Hierarchical Attention}

Let $\mathcal{A}$ be any algorithm that maps hierarchical token structures to attention patterns. We define the following axioms that any reasonable hierarchical attention mechanism should satisfy:

\begin{axiom}[Implementation Invariance]
For any two functionally equivalent implementations of the same hierarchical structure, the attention patterns must be identical:
\[
\forall H_1, H_2: \text{if } H_1 \equiv H_2 \text{ then } \mathcal{A}(H_1) = \mathcal{A}(H_2)
\]
\end{axiom}

\begin{axiom}[Sensitivity]
If a token $x$ depends semantically on token $y$, then the attention mechanism must reflect this dependency:
\[
\text{dep}(x,y) \implies \exists l: \text{att}_l(x,y) > 0
\]
where $\text{att}_l(x,y)$ represents the attention score from $x$ to $y$ in layer $l$.
\end{axiom}

\begin{axiom}[Completeness]
The attention patterns must fully capture the hierarchical structure:
\[
\forall x,y \in T: \sum_{l=1}^L \text{att}_l(x,y) = \mathcal{M}(x,y)
\]
where $\mathcal{M}(x,y)$ is the hierarchical mask defined by token levels.
\end{axiom}

\begin{axiom}[Structural Preservation]
The attention mechanism must preserve the categorical structure through a functor $F: \mathcal{H} \rightarrow \mathcal{A}$ satisfying:
\begin{itemize}
    \item Composition: $F(f \circ g) = F(f) \circ F(g)$
    \item Order: $a \leq_{\mathcal{H}} b \implies F(a) \leq_{\mathcal{A}} F(b)$
    \item Isomorphism: $\exists \eta: 1_{\mathcal{H}} \Rightarrow F^{op}F$ with coherence
\end{itemize}
\end{axiom}

\subsubsection{Uniqueness Theorem}

\begin{theorem}[Uniqueness of Hierarchical Attention Structure]
Any attention mechanism $\mathcal{A}$ satisfying Axioms 1-4 must be structurally equivalent to our proposed algorithm.
\end{theorem}

\begin{proof}
Let $\mathcal{A}$ be any algorithm satisfying the axioms. We prove structural uniqueness through two key aspects:

\textbf{Step 1: Level Assignment Uniqueness}

First, we show that the hierarchical level assignment must be identical. Consider any token $t$ in the input:

\begin{itemize}
    \item By Implementation Invariance, the level assignment must be independent of how the token is represented
    \item By Sensitivity, if $t$ depends on any token $s$, then $\text{level}(t) \geq \text{level}(s)$
    \item By Completeness, every token must be assigned exactly one level
\end{itemize}

Therefore:
\[
\text{level}_{\mathcal{A}}(t) = \argmin_{l} \{\text{level}(t) \geq \text{level}(s) \text{ for all } s \text{ that } t \text{ depends on}\}
\]

This is exactly the level assignment used in our algorithm, proving:
\[
\text{level}_{\mathcal{A}}(t) = \text{level}_{\text{our}}(t) \text{ for all tokens } t
\]

\textbf{Step 2: Attention Pattern Structure}

Next, we prove that the structure of attention patterns must be identical. Let $x, y$ be any pair of tokens:

1. By Structural Preservation (Order), we have:
\[
\text{level}(x) \leq \text{level}(y) \implies \text{att}_{\mathcal{A}}(x,y) \text{ is allowed}
\]

2. By Completeness:
\[
\sum_{l=1}^L \text{att}_{\mathcal{A},l}(x,y) = \mathcal{M}(x,y)
\]
where $\mathcal{M}(x,y)$ is our hierarchical mask.

3. By Structural Preservation (Composition):
\[
\text{att}_{\mathcal{A}}(x,z) = \sum_{y} \text{att}_{\mathcal{A}}(x,y) \cdot \text{att}_{\mathcal{A}}(y,z)
\]
when there exists a compositional path $x \rightarrow y \rightarrow z$.

These conditions force:
\[
\text{att}_{\mathcal{A}}(x,y) = \begin{cases}
    \mathcal{M}(x,y) & \text{if } \text{level}(x) \leq \text{level}(y) \\
    0 & \text{otherwise}
\end{cases}
\]

\textbf{Conclusion}

The combination of these steps shows that:
\begin{enumerate}
    \item The level assignment is uniquely determined
    \item The attention pattern structure is uniquely determined
\end{enumerate}

Therefore, any algorithm $\mathcal{A}$ satisfying our axioms must produce structurally equivalent attention patterns to our algorithm.
\end{proof}

==> sections/08_tables.tex <==
% Table 1: miniF2F Results
\begin{table}[t]
\begin{center}
\caption{Results on miniF2F benchmark. Pass@K denotes the percentage of theorems successfully proved with K = 1 × 32 × 100 attempts. Complexity shows the average number of proof steps, and Ratio represents the relative complexity compared to baseline.}
\label{tab:minif2f_results}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Pass@3200 (\%)} & \multicolumn{2}{c}{Complexity} & \multicolumn{2}{c}{Ratio} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& Test & Valid & Test & Valid & Test & Valid \\
\midrule
Baseline & 29.51 & 31.55 & 1.89 & 3.11 & 1.00 & 1.00 \\
Ours & \textbf{31.15} & \textbf{34.02} & \textbf{1.67} & \textbf{2.00} & \textbf{0.88} & \textbf{0.64} \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

% Table 2: ProofNet Results
\begin{table}[t]
\begin{center}
\caption{Results on ProofNet benchmark. Pass@K denotes the percentage of theorems successfully proved with K = 1 × 32 × 100 attempts. Complexity shows the average number of proof steps, and Ratio represents the relative complexity compared to baseline.}
\label{tab:proofnet_results}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Pass@3200 (\%)} & \multicolumn{2}{c}{Complexity} & \multicolumn{2}{c}{Ratio} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& Test & Valid & Test & Valid & Test & Valid \\
\midrule
Baseline & 13.56 & 9.04 & 1.83 & 2.00 & 1.00 & 1.00 \\
Ours & \textbf{14.69} & \textbf{10.73} & \textbf{1.83} & \textbf{1.00} & \textbf{1.00} & \textbf{0.50} \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
